Adversarial Dueling Bandits

We introduce the problem of regret minimization in Adversarial Dueling Bandits. As in classic Dueling Bandits, the learner has to repeatedly choose a pair of items and observe only a relative binary `win-loss' feedback for this pair, but here this feedback is generated from an arbitrary preference matrix, possibly chosen adversarially. Our main result is an algorithm whose $T$-round regret compared to the \emph{Borda-winner} from a set of $K$ items is $\tilde{O}(K^{1/3}T^{2/3})$, as well as a matching $\Omega(K^{1/3}T^{2/3})$ lower bound. We also prove a similar high probability regret bound. We further consider a simpler \emph{fixed-gap} adversarial setup, which bridges between two extreme preference feedback models for dueling bandits: stationary preferences and an arbitrary sequence of preferences. For the fixed-gap adversarial setup we give an $\smash{ \tilde{O}((K/\Delta^2)\log{T}) }$ regret algorithm, where $\Delta$ is the gap in Borda scores between the best item and all other items, and show a lower bound of $\Omega(K/\Delta^2)$ indicating that our dependence on the main problem parameters $K$ and $\Delta$ is tight (up to logarithmic factors).

==> alg_fxdgap_tk.tex <==
\section{Algorithm: \prob~ with \gap \,($\Delta$)}
\label{sec:alg_fxdgap}

\paragraph{Setup.} \tk{setup should move to preliminaries}
We first consider an `\emph{easier setup}' which an additional assumption on the sequence of preference matrices $\{\P_t\}_{t = 1}^T$. More formally we assume that $~\exists i^* \in [K] \forall t \in [T]$ such that $\bar b_t(i^*) > \bar b_t(j) + \Delta, \forall j \in [K]\sm\{i^*\}$, where we denote by $\bar b_t(i) := \frac{1}{t}\sum_{\tau = 1}^t b_\tau(i)$, the average \emph{borda score} of any item $i \in [K]$ at time $t$.
We denote the above problem setup as \acrgap$(K,T,\Delta)$.


\textbf{Algorithm: Key Ideas. } Our algorithm \red{to be added...}

%We define for each action $i \in [K]$ a lower confidence borda score $LCB(i;t)=\ts_t(i) - \sqrt{\frac{\log T/\delta}{n_i(t)}}$, and an upper confidence borda score $UCB(i;t)=\ts_t(i) + \sqrt{\frac{\log T/\delta}{n_i(t)}}$. 

\begin{center}
\begin{algorithm}[H]
   \caption{\textbf{\alggap \, (BCB)}}
   \label{alg:gap}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} ~~ Item set: $[K]$%, learning rate $\eta > 0$, parameters $\gamma \in (0,1)$ %scale parameter $\lambda_t$
   %\STATE \quad\quad\quad\quad Confidence parameter: $\delta >0$
   \STATE {\bfseries Initialize:} Candidate set $\cC_1 \leftarrow [K]$, $t \leftarrow 1$ %$n_0(i) \leftarrow 0$, $\tb_0(i) \leftarrow 0$, $\forall i \in [K]$.
   \WHILE {$|\cC_t|\geq 2$}
   \STATE Select $x_t \in \cC_t$ uniformly at random. Select $ y_t \in [K]\sm\{x_t\}$ uniformly at random.
   \STATE Receive preference $o_{t}(x_t,y_t) \sim \text{Ber}(\P_t(x_t,y_t))$
   %\STATE $n_{t}(x_t) \leftarrow n_{t-1}(x_t)+1$, $n_{t}(i) \leftarrow n_{t-1}(i), ~\forall i \in [K]\sm\{x_t\}$
   \STATE Estimated score: $\hb_{i}(t) = \frac{\1(x_t = i)}{1/|\cC_t|}o_t(x_t,y_t), ~\forall i \in \cC_t$		
   \STATE $\tb_{t}(i) \leftarrow \frac{1}{t}\sum_{\tau = 1}^t\hb_{\tau}(i)$, $\forall i \in \cC_t$
   \STATE $LCB(i;t) = \tb_t(i) - \sqrt{\frac{4|\cC_t|\log (2KT/\delta)}{t}}$, $UCB(i;t) = \tb_t(i) + \sqrt{\frac{4|\cC_t| \log (2KT/\delta)}{t}}$
   \STATE $\cC_{t+1} \leftarrow \cC_t \sm \{j \in \cC_t \mid \exists  i \in \cC_t$ s.t. $LCB(i;t)> UCB(j;t) \}$
   \STATE $t=t+1$
   \ENDWHILE
   \STATE Assuming $\cC_t =\{\hat{i}\}$, play $(\hat i,\hat i)$ for rest of the rounds $t, t+1, \ldots, T$. 
\end{algorithmic}
\end{algorithm}
\vspace{-2pt}
\end{center}

We now proceed to the proving regret guarantee of \alggap \, (Alg. \ref{alg:gap}) in Thm. \ref{thm:ub_gap_whp}. 
Let us first abbreviate $o_t(x_t,y_t)$ as $o_t$, and denote by $\cH_{t-1} := \sigma(\P_1,(x_1,y_1),o_1, \ldots,\P_t)$ be the history (sigma algebra of the past information) available till time $t$, which does not include the randomness of players action $(x_t,y_t)$ at time $t$ and hence that of $o_t$. 

\begin{restatable}[High Probability Regret Guarantee: \alggap]{thm}{ubdgap}
\label{thm:ub_gap_whp}
Given any $\delta>0$, with probability at least $(1-\delta)$, the regret incurred by \alggap ~(Alg. \ref{alg:gap}) for the problem of \acrgap$(K,T,\Delta)$ can be upper bounded as:
\[
   R_T 
   \leq 
   \frac{4K \log (K T/ \delta)}{9} + \frac{64 K\log (2KT/\delta)}{\Delta^2}
   .
\]
\end{restatable}

The proof relies on the the following two key lemmas:

\begin{restatable}[Unbiased Estimate of the Borda Score]{lem}{estbordagap}
\label{lem:est_borda_gap}
For any fixed $n > 0$, let 
At any round $t \in [T]$, we have  $\E_{\cH_t}\Big[\tb_{t}(i) \Big] = \bb_{t}(i)$ for any $i \in \cC_t$. 
\end{restatable}

\begin{restatable}[High Probability Confidence Bounds on Estimated-Borda Scores]{lem}{gapconf}
\label{lem:gap_conf}
For any item $i \in \cC_t$, for all round $t > \frac{4K \log (K T/ \delta)}{9}$, with probability at least $(1-\delta)$, $\bb_i(t) \in [LCB(i;t),UCB(i;t)]$. In other words 
\[
Pr\big(\exists i \in \cC_t, \forall t > \frac{4K \log (K T/ \delta)}{9} \text{ s.t. } \bb_i(t) \notin [LCB(i;t),UCB(i;t)] \big) < \delta.
\] 
\end{restatable}

\begin{proof}[Proof (sketch)]
The proof now follows .... \red{to be added...}
\end{proof}


\begin{rem}
\label{rem:thm_gap}
\red{comment on optimality}
\end{rem}

==> lemma14-sketch-ym.tex <==

\textbf{{Proof (sketch).}} 
The proof relies on constructing a `hard enough' problem instance for the learning framework and showing no algorithm can achieve a smaller rate of regret on that instance than the claimed lower bounds.
%
For simplicity of notation we assume $K$ is even and denote by $\tK:= \frac{K}{2}$. 
%
Let us construct $\tK+1$ problem instances $\cI^1,\cI^2,\ldots,\cI^\tK$ and $\cI^0$, where each instance is uniquely identified by its underlying preference matrix as defined below: 

\noindent \textbf{Problem instance}$(\cI^0)$: For all $t \in [T]$, $P_t(i,j) = 
\begin{cases} 
0.5,~\forall i,j \in [\tK]$ \text{ or } $i,j \in [K]\sm [\tK]\\
0.9,~\forall i \in [\tK]$ \text{ and } $\forall j \in [K]\sm [\tK]\\
\end{cases}
$.

Note for $\cI^0$, $\forall t \in [T]$, for any item $i \in [\tK]$, $s_t(i) = 0.7$, and for any item $i \in [K]\sm[\tK]$, $s_t(i) = 0.3$. 
Thus for the instance $\cI^0$, any item $i \in [\tK]$ is an optimal arm. Now let us consider $\tK$ alternative problem instances $\cI^{m} ~~\forall m \in [\tK]$:

\noindent \textbf{Problem instance}$(\cI^{m})$: 
For all $t \in [T]$, $P_t(i,j) = 
\begin{cases} 
0.5,~\forall i,j \in [\tK]$ \text{ or } $i,j \in [K]\sm [\tK]\\
0.9,~\forall i \in [\tK]$ \text{ and } $\forall j \in [K]\sm [\tK]\\
0.9+\epsilon,~\text{if } i = m, \forall j \in [K]\sm [\tK]
\end{cases}
$,  
for some $\epsilon\in (0,0.1]$.
%
Note for any $\cI^{m}$, $\forall t \in [T]$, for any item $s_t(i) = 
\begin{cases}
0.7 , ~\forall i \in [\tK]\sm\{m\}\\
0.7+\epsilon, \text{ if } i = m\\
0.3-\frac{\epsilon}{K}, \text{ if } i = n
\end{cases}
$. 

Clearly, for instance $\cI^{m}$, the unique \emph{`best'} item is $i^{m}_{*}:=m$, and all $j \in [K]\sm[tK]$ items are the \emph{`bad'} playing which at any round $t \in [T]$ yields a  constant regret of $\frac{\big(s_t(i^{m}_{*}) - s_t(j)\big)}{2} = 0.2 + \frac{(K+1)\epsilon}{2K}$, and all $j \in [\tK]\sm\{m\}$ items are the \emph{`near-best'} playing which at any round $t \in [T]$ yields at least a regret of $\frac{\big(s_t(i^{m}_{*}) - s_t(j)\big)}{2} = \frac{\epsilon}{2}$. %However in order to distinguish the \emph{`best'} and the \emph{`near-best'} items, it is necessary to play the \emph{`bad'} items `sufficiently enough' to infer which of the $[\tK]$ items has the highest borda score. Intuitively the main idea of our lower bound technique lies in showing that in this process any learner has to pull the \emph{`bad'} items \emph{at least} a certain number of times which would lead consequently lead to the regret lower bound. The remaining arguments proves this formally. 
%to show a regret of at least $\Omega(K^{1/3}T^{2/3})$. 

Let us define $N_T(i,j) := \E[\sum_{t = 1}^T\1(\{i,j\} = \{x_t,y_t\})]$, the number of times algorithm pulls arm-pair $(i,j) \in [K]\times[K]$ in $T$ rounds. 
%
%For simplicity of notations, we henceforth would denote $N^{\cA}_T(\cdot) = N_T(\cdot)$. 
We also denote by $D_t = \{x_t,y_t\}$, and $\Delta^{m}_j = \frac{\big(s_t(i^m_*) - s_t(j)\big)}{2}$, for all $m \in [\tK],~ j \in [K]$.
%
%We now make the following two key observations:
%\textbf{Observation $1$.} We consider only the class of all deterministic algorithms, i.e. where $x_t,y_t$ is a deterministic function of the past history $\cH_{t-1}$. Note this is without loss of generality, since any randomized strategy can be seen as a randomization over deterministic querying strategies. Thus, a lower bound which holds uniformly for any deterministic class of algorithms, would also hold over a randomized class of algorithms.
%
%\textbf{Observation $2$.} We also consider that for any instance $\cI^m$ ($m \in [\tK]\cup\{0\}$), the algorithm $\cA$ pulls the `suboptimal-pairs' (i.e. any pair which contains at least one bad arm from $[K]\sm[\tK]$) for at most $\epsilon T$ times, i.e. for any $m \in [\tK]\cup\{0\}$, $\E_{\cI^{m}}[\sum_{i,j \mid \{i,j\} \cap [K]\sm[\tK] \neq \emptyset} N^{\cA}_T(i,j)] \le \epsilon T$. \red{This indeed is without loss of generality since ... ... Clarify properly.}
%for any `bad' item $j \in [K]\sm[\tK], ~ \Delta^m_j \ge 0.2 = O(1)$, i.e. the learner incurs a constant regret and  for any `near-best' item $j \in [\tK]\sm\{m\}, ~ \Delta^m_j = \frac{\epsilon}{2}$.
%  
We will break the analysis into two cases:
%$(1).\, T \le \frac{K}{1440 \epsilon^3}$, and $(2).\, T > \frac{K}{1440 \epsilon^3}$. 

\textbf{Case 1. \big($T \le \frac{K}{1440 \epsilon^3}$\big):} 
For simplicity we first prove a lower bound on 
$R_T^s$ defined in terms of the \emph{`shifted-borda score'} $s_t$ (Rem. \ref{rem:regeqv}).
We first prove that the regret of any algorithm $\cA$ on instance $\cI^{m}$ for $T$ rounds, can be lower bounded as: 

\vspace{-18pt}
\begin{align*}
\nonumber \E_{\cI^{m}}[R_T^s(\cA)] \ge \frac{\epsilon}{2}\Bigg(T - \bigg(\frac{\sum_{m \in [\tK]}\E_{\cI^{0}}[N_T(m,m)]}{\tK} + T\sqrt{\Big(  \frac{1}{2\tK}\sum_{m \in [\tK]}D_{KL}(\cI^0,\cI^{m})\Big)}\bigg) \Bigg).
%\vspace{-5pt}
\end{align*}
%
where $D_{KL}(\cI^0,\cI^{m})$ denotes the KL-divergence between the probability distribution induced on the observed history $\cH_T$ by the problem instance $\cI^0$ and $\cI^{m}$. Further using chain rule of KL-divergence with few more observations we show that:
$%\begin{align*}
\frac{\sum_{m \in [\tK]}D_{KL}(\cI^0,\cI^{m}) }{\tK}  \le \frac{90\epsilon^3 T}{\tK}
$. %\end{align*}
%
Combining the above two crucial results we obtain:

\begin{align*}
%\label{eq:lb0}
\E [R_T^s(\cA)] \ge \frac{\epsilon}{2}\big(T - \big(\frac{T}{\tK} + T\sqrt{\big(\frac{90\epsilon^3 T}{K}\big)}\big) \big)
\overset{(1)}{\ge} \frac{\epsilon}{2}\big(T - \big(\frac{2T}{K} + T\sqrt{\frac{1}{16}}\big) \big) \ge \frac{\epsilon}{2}\big( T - \frac{3T}{4} \big) = \frac{\epsilon T}{8}
\end{align*}
where $(1)$ holds since by the assumption of Case \textbf{1} we have $T \le \frac{K}{1440 \epsilon^3}$, and the last inequality follows for any $K \ge 4$. This gives a regret lower bound for Case \textbf{1}.

\textbf{Case 2. \big($T > \frac{K}{1440 \epsilon^3}$\big):}
For this case we show for any $T' > T_0$ it has to be the case that $R^s_{T'} \ge \Omega\Big(\frac{K}{\epsilon^2}\Big)$, as otherwise it would lead to a contradiction for the lower bound result obtained in case \textbf{1}. 
The final regret lower bound follows by combining the lower bounds of Case \textbf{1} and \textbf{2}, and from the fact that $R_T \ge {R_T^s}$ (as per Rem. \ref{rem:regeqv}). 
%
The complete proof is given in Appendix \ref{app:lb}.
\hfill $\square$

